How Firms Adapt and Interact in Open Source Ecosystems: Analyzing Stakeholder Influence and Collaboration Patterns

[Context and motivation] Ecosystems developed as Open Source Software (OSS) are considered to be highly innovative and reactive to new market trends due to their openness and wide-ranging contributor base. Participation in OSS often implies opening up of the software development process and exposure towards new stakeholders. [Question/Problem] Firms considering to engage in such an environment should carefully consider potential opportunities and challenges upfront. The openness may lead to higher innovation potential but also to frictional losses for engaged firms. Further, as an ecosystem progresses, power structures and influence on feature selection may fluctuate accordingly. [Principal ideas/results] We analyze the Apache Hadoop ecosystem in a quantitative longitudinal case study to investigate changing stakeholder influence and collaboration patterns. Further, we investigate how its innovation and time-to-market evolve at the same time. [Contribution] Findings show collaborations between and influence shifting among rivaling and non-competing firms. Network analysis proves valuable on how an awareness of past, present and emerging stakeholders, in regards to power structure and collaborations may be created. Furthermore, the ecosystem's innovation and time-to-market show strong variations among the release history. Indications were also found that these characteristics are influenced by the way how stakeholders collaborate with each other.

==> 03_Case_Study_Design.tex <==
\section{Case Study Design}
% By analyzing how stakeholder influence and collaborations fluctuate over time we aim to investigate how firms adapt and interact inside open source ecosystems. By further investigating the impact of these patterns on the degree of innovation and time-to-market of a release, the goal is to provide decision support for engaged firms and input to their product planning and contribution strategies. Case study was chosen as research strategy due to our wish for an exploratory approach with a flexible research design~\cite{runeson2009guidelines}.

% \subsection{Research Questions}
% To adress the rationale and goal of this paper the following research questions was defined in context of the Apache Hadoop ecosystem:

% \begin{enumerate}[RQ1]
% %\item What are the business models and relationships of top stakeholders in the Apache Hadoop ecosystem?
% \item How does the time to market and the degree of innovation evolve over time?
% \item How does stakeholder influence and collaboration evolve over time? 
% \item How does stakeholder influence affect number of its reported issues included in a release?
% \item Does stakeholder influence and collaboration impact the time to market and the degree of innovation? 
% \end{enumerate}


\subsection{Case Selection and Units of Analysis}\label{sec:unitOfAnalysis}
Apache Hadoop is an open source software framework, which other applications may use to distribute and parallelize processing of large data sets over scalable clusters of computers. This includes both computation and storage locally on the machines. The framework consists of four modules:
\begin{itemize}
\item Hadoop Common - Common functionality and utilities used by other modules.
\item Hadoop Distributed File System (HDFS) - A distributed file system providing high throughput between machines in a cluster. 
\item Hadoop YARN - Framework for managing and scheduling resources and user applications across a cluster.
\item Hadoop MapReduce - A programming model for processing of large data sets.
\end{itemize}

Apache Hadoop is part of an ecosystem with the same name, which includes software that builds on top of the framework. Several other Apache projects are included in this ecosystem, e.g. Apache Spark, Apache HBase, Apache Pig and Apache Hive. Apache Hadoop was launched as an Apache project in 2006 after initial development at Yahoo!. Today its users include large firms such as Microsoft, Amazon, Google, LinkedIn, Twitter and Facebook.

%\todo[inline]{Development/release process?}

%\todo[inline]{Data demographics: number of projects (4), artifact types, number of artifacts instances, types of contributors/stakeholders, number of stakeholders per type, number of releases, time span of the project, }

Apache Hadoop was chosen from a subset of Apache open source projects as single case in an embedded case study~\cite{runeson2009guidelines} due to the community's strict contribution process. A second reason was due to the composition of the community as most contributors have a corporate affiliation.

To create a longitudinal perspective and comparison of the data, issues were analysed in sets reflecting the release cycles. Due to the complicated release history of Apache Hadoop, the selection of releases were narrowed down to sub releases, spanning from 2.2.0 (released 15/Oct/13) to 2.7.1 (06/Jul/15), thus constituting the units of analysis through the study. Third level releases were aggregated into their parent upper level release.

Issues were furthermore chosen as the main data source as these can be connected to a specific release. To determine who collaborated with who over an issue, attachments submitted by each stakeholder were used. This is because users who wish to contribute work to an issue have to package their code into a patch and then attach it to the issue in question. After having been approved by the automated tests and a code reviewer, a commiter may then choose to commit it.

==> 04_Methodology.tex <==
\section{Methodology}

The following steps were performed, see Fig. X.
\todo[inline]{Create picture}

\begin{enumerate}
\item Decision on unit of analysis.
\item Data collection through crawling of issue database.
\item Indexing and restructuring of data in a relational database.
\item Exploratory analysis with SNA and R.
% \item Confirmatory and exploratory interviews with two committers.
\item Synthesis of findings.
\end{enumerate}

\subsection{Data Collection}
The issue data was stored in a JIRA Issue Tracker used by the Apache Hadoop community. A crawler was implemented to collect, parse and index the data into a relational database. Database schema was inspired by that used in Bicho\footnote{https://github.com/MetricsGrimoire/Bicho}, another tool for crawling issue repositories. 

To determine organizational affiliation, the domin of the issue authors' email addresses were used. Where affiliation could not be determined (e.g. for gmail-addresses) secondary sources were used such as LinkedIn and Google where the issue authors full name functioned as keyword.

\subsection{Data Analysis}
Attachment data correlating to the issues belonging to each release were used as input to the SNA process. Two authors were paired when they each had submitted at least one attachment to the same issue. Based on the affiliation, pairs were aggregated and abstracted to an organizational level. 

% \subsubsection{Edge weights:}
A directed network was constructed with vertices representing the organizations, i.e. the stakeholders. As suggested by Orucevic et al.~\cite{orucevic2014network} weights are calculated to describe the strength of the relationships constituted by the directed edges. Instead of counting single number of attachments however, we wish to consider the size of the stakeholders contributions relative each other further. This is done by addressing the net changed lines of code (LOC) per attachment, i.e. number of added lines minus number of deleted lines.

For example, see Fig.~\ref{fig:NetworkExample}. Stakeholders A, B and C have all contributed one attachment each to the same issue. A's attachment contains 100 added LOC and 50 deleted LOC, resulting in a net of 50 added LOC. B's attachment contains a net of 100 added LOC, while C's attachment contains a net of 150 added LOC. In total 300 LOC has been suggested to the issue. Hence, the weighted influence from A becomes 50/300, 100/300 from B and 150/300 from C.

\begin{figure*}[hbtp]
\centering
\includegraphics[scale=.3]{NetworkExample.PNG}
\caption{Example of a weigthed network between three stakeholders that's contributed attachment to the same issue(s).}
\label{fig:NetworkExample}
\end{figure*}

Adopted from Orucevic et al.~\cite{orucevic2014network}, and given a set of stakeholders $V = \{v_{1}, v_{2},.., v_{k}\}$ and a set of collaborations $U = \{u_{1}, u_{2},.., u_{k}\}$, we formally define the edge weight $W$ from a certain stakeholder $v_{i}$ to all other stakeholders who are active in the collaboration of an issue $u_{t}$ as:

$$W\left ( v_{i}, v_{j}, u_{t}  \right ) = \frac{X\left ( v_{i}, u_{t} \right )}{\sum_{c=1}^{k} X\left ( v_{c}, u_{t} \right )}$$

where $X\left ( v_{i}, u_{t} \right )$ is the net amount of LOC in the attachment(s) added to the issue $c_{t}$ by stakeholder $v_{i}$. By accumulating this weight over all collaborations on issues $u_{t}$ between stakeholder $v_{i}$ and $v_{j}$ the final edge weight may be defined as:

$$W\left ( v_{i}, v_{j}  \right ) = \sum_{t=1}^{m} W\left ( v_{i}, v_{j}, u_{t}  \right )$$


\subsubsection{Network Analysis}
For the analysis R was used together with the TNet package due to that it can consider weighted edges. Gephi was used to visualize the network graphs. The following metrics were used:

% \subsubsection{Software used:}
% For the analysis R was used together with packages TNet and iGraph. TNet was used to calculate the metrics needed and was chosen due to that it can consider weighted edges. iGraph and Gephi was used to visualize the network graphs.

% \subsubsection{Metrics:}
% Three network centrality metrics and two network overview metrics were used, described below respectively.

\begin{itemize}
\item \textit{Weighted Outdegree Centrality} - In a directed graph, outdegree is the number of outgoing ties from one vertex to others. For weighted networks, the sum of all outgoing edges' weights results in the node strength, labeled forward as outdegree centrality. Higher index indicates higher influence on its neighbours.
\item \textit{Betweeness Centrality} - This metric describes how central a vertex is by considering number of shortest paths between any two other vertices that passes through the vertex in question. Higher index indicates higher importance.
\item \textit{Closeness Centrality} - Indicates an average relative distance to all other nodes in the network based on the shortest paths. Higher index indicates that a vertex is well related and have better possibilities in spreading information in the network.
\item \textit{Average Clustering Coefficient} - Indicates how likely it is that there will form clusters in the network.
\item \textit{Graph Density} - A measure of many edges that are present in relation to the total number of possible edges. Indicates how complete in connections the networks is.
\end{itemize}



% \subsection{Interviews}
% Interviews were performed after the quantitative data analysis to give further input to initial findings and for the researchers to have a better understanding of the case. A subset of potential interviewees were contacted among the members of the governance board of Apache Hadoop. Care was taken to only elicit one interviewee per firm. Two interviewees answered and were interviewd in a semi-structured manner with a protocol partly based on initial findings from the quantitative analysis. Interviews were later transcribed, decoded thematically~\cite{Cruzes14} and synthesized with earlier findings.

==> 07_Threats_To_Validity.tex <==
\vspace{-0.4cm}
\section{Threats to Validity}\label{sec:threats}
\vspace{-0.3cm}

Four aspects of validity in regards to a case study are \textit{construct}, \textit{internal} and \textit{external validity}, and \textit{reliability}~\cite{runeson2009guidelines}. 

In regards to \textit{construct validity}, one concern may be definition and interpretation of network metrics. The use of weights to better represent a stakeholders' influence, as suggested by Orucevic-Alagic et al.~\cite{orucevic2014network} was used with the adoption to consider the net of added LOC to further consider the relative size of contributions. A higher number of LOC however does not have to imply increased complexity. We chose to see it as a simplified metric of investment with each LOC representing a cost from stakeholder. Other options could include consideration software metrics such as cyclomatic complexity. With the weights considered, the metrics together offers an understanding a stakeholder's importance in an ecosystem may be created. Network metrics excluded, e.g. the eigenvector centrality and the clustering coefficient could offer further facets.

Furthermore, we focused on input (number of issues) and output (implementation change size) related metrics \cite{knight2005metrics} for operationalizing the innovation per release. Future studies could additionally include process related metrics. Release cycle times were used for quantifying the time-to-market as suggested by Griffin~\cite{griffin1993metrics}. Since we solely analyzed releases from the time where the Apache Hadoop ecosystem was already well established, a potential drawback is that a long requirements analysis ramp up time may not be covered by this measure.

A threat to \textit{internal validity} concerns the observed correlation of how the time-to-market and the innovativeness of a release is influenced by the way how stakeholders collaborate with each other. This needs further replication and validation in future work.

In regards to \textit{external validity}, this is an exploratory single case study. Hence observations need validation and verification in upcoming studies in order for findings to be further generalized. Another limitation concerns that only patches of issues were analyzed. In future work, consideration should also be taken to comments for example as this may also be an indicator of influence and collaboration. Further, number of releases in this study was limited due to a complicated release history in the Apache Hadoop project, but also a design choice to give a further qualitative view of each release in a fine-grained time-perspective. Future studies should strive to analyze longer periods of time.

Finally, in regards to \textit{reliability} one concern may be the identification of stakeholder affiliation. A contributor could have used the same e-mail but from different roles, e.g. as an individual or for the firm. Further, sources such as LinkedIn may be out of date.

